High-Dimensional Bayesian Optimization via Additive Models with Overlapping Groups

Bayesian optimization (BO) is a popular technique for sequential black-box function optimization, with applications including parameter tuning, robotics, environmental monitoring, and more. One of the most important challenges in BO is the development of algorithms that scale to high dimensions, which remains a key open problem despite recent progress. In this paper, we consider the approach of Kandasamy et al. (2015), in which the high-dimensional function decomposes as a sum of lower-dimensional functions on subsets of the underlying variables. In particular, we significantly generalize this approach by lifting the assumption that the subsets are disjoint, and consider additive models with arbitrary overlap among the subsets. By representing the dependencies via a graph, we deduce an efficient message passing algorithm for optimizing the acquisition function. In addition, we provide an algorithm for learning the graph from samples based on Gibbs sampling. We empirically demonstrate the effectiveness of our methods on both synthetic and real-world data.

==> title.tex <==
\begin{titlepage}
\vfill
\begin{center}
\includegraphics{Figure/EPFL}
\vfill
\huge
\textsc{High Dimensional Bayesian Optimisation via Additive Kernel Learning}\\
\vspace{.5cm}
\LARGE
Paul Rolland\\
\vfill
\large
Professor: Volkan Cevher \\
Supervisors : Ilija Bogunovic, Jonathan Scarlett\\
\vfill
\end{center}
\vspace*{0.5cm}
%noindent
{\bf Abstract: } Black-box function optimisation is a widely studied problem that aims at optimising a black-box function via point evaluations. A popular algorithm for performing this task selects the next point to evaluate based on a posterior estimation of the target function conditioned on the observations. This is known as Bayesian Optimisation (BO). The function to optimise can potentially be high dimensional, and this task becomes exponentially harder as the dimension increases. We base our work on a popular setting for scaling high dimensional BO, which models the target function as a sum of low dimensional independent components. This was proposed by Kandasamy et al.~\cite{conf/icml/KandasamySP15}, but they constrained the terms in the decomposition to be fully independent from each other, and thus restricted the dependency graph to blocks of disjoint fully connected components. In this project, we remove this assumption and design an algorithm for handling any dependency graph. The main challenge is to efficiently optimise the acquisition function over the high dimensional space. This challenge is resolved by appropriately defining the acquisition function, and by using a message-passing algorithm on the dependency graph in order to optimise it. We also provide an efficient way of learning the structure of the dependency graph, based on Gibbs sampling and maximum likelihood approach. We empirically demonstrate the benefit of this method on synthetic data and provide a real face detection example in which our model outperforms the constrained additive BO model. Finally, we discuss the issues in proving theoretical guarantees for our method, and provide theoretical bound for the maximum information gain.
\vspace*{0.5cm}
\begin{center}
\vfill
\large
\today
\normalsize
\end{center}
\end{titlepage}
